Practical Superdirective and Efficient Rectenna for Low-Power RF Energy Harvesting

This paper presents the design and analysis of a superdirective rectenna optimized for enhanced RF-to-DC efficiency and realised gain, featuring direct impedance matching between the antenna and the rectifier. Employing passively loaded, low profile strip dipoles on a low-loss substrate, the rectenna achieves a realised gain of 6.9 dBi and an RF-to-DC efficiency of 22.1% at -20 dBm.

==> Figs/myantennageom001.tex <==
\def\myLa{1.75}
\def\myWa{6}
\def\myLb{2}
\def\myWb{3}
\def\myD{1.5}
\def\myB{1.7}
\def\myG{0.275}
\def\myI{0.5}
\def\myLeg{0.5}
\def\myLegOff{1.0}
\def\myVs{1.5}
\def\myC{5}

\ctikzset{
	amplifiers/fill=cyan,
	sources/fill=white,
	diodes/fill=red,
	resistors/fill=violet,
}

\begin{circuitikz}
	\coordinate (start) at (0,0);
	\coordinate (P) at (\myD,\myB);
	\coordinate (A) at (\myD,-\myB*0.8);
	\coordinate (B) at (0,-\myB*0.8);
	%
	\draw[line width=0.5pt, rounded corners, color=black, -]
	(start) -- ++(0.75*\myD,0);
	\draw[line width=0.5pt, rounded corners, color=black, ->]
	(start) ++(1.125*\myD,0) -- ++(0.6*\myD,0) node[right] {$x$};
%	\draw[line width=0.5pt, rounded corners, color=black, ->]
%	(start) -- ++(0,1.5*\myLa) node[above] {$z$};
	%
	\draw[line width=\myWa pt, rounded corners, color=myblue]
	(start)++(0,\myG) -- (0,\myLa)
	(start)++(0,-\myG) -- (0,-\myLa);
	%
	\draw[line width=\myWb pt, rounded corners, color=myblue]
	(start)++(\myD,\myG) -- (\myD,\myLb)
	(start)++(\myD,-\myG) -- (\myD,-\myLb)
	%
	;
%	\draw[line width=0.35pt, rounded corners, color=black, - ]
%	(start) -- (P) node[midway, above] {$r_c$}
%	node[right] {$E(z)$}
%	(start)++(0,-\myLa) -- (P) node[midway, left] {$r_b$}
%	(start)++(0,\myLa) -- (P) node[midway, above] {$r_a$};
	%
%	\draw[line width=0.5pt, rounded corners, color=black, ->]
%	(A)++(0,-\myI/2) -- ++(0,\myI) node[midway, left] {$I_2(z)$};
%	\draw[line width=0.5pt, rounded corners, color=black, ->]
%	(B)++(0,-\myI/2) -- ++(0,\myI) node[midway, left] {$I_1(z)$};
	%
	\draw[line width=0.5pt, rounded corners, color=black, Bar-Bar ]
	(start)++(-1.0*\myLegOff,-\myLa) -- ++(0,2*\myLa) node[midway, left] {$L_1$};
	\draw[line width=0.5pt, rounded corners, color=black, Bar-Bar]
	(start)++(\myD+1.0*\myLegOff,-\myLb) -- ++(0,2*\myLb) node[midway, above right] {$L_2$};
	%
	\draw[line width=0.5pt, rounded corners, color=black, Bar-Bar]
	(start)++(-\myWa/2 pt,-\myLa-\myLegOff/2) -- ++(\myWa pt,0) node[right] {$w_1$};
	\draw[line width=0.5pt, rounded corners, color=black, Bar-Bar]
	(start)++(\myD cm -\myWb/2 pt,-\myLa-\myLegOff/2/0.9) -- ++(\myWb pt,0) node[right] {$w_2$};
	\draw[line width=0.5pt, rounded corners, color=black, Bar-Bar]
	(start)++(0,-\myLb-\myLegOff*0.9) -- ++(\myD,0) node[midway, above] {$d$};
	%
	\draw 
	(start)++(-0*\myLegOff/2,-1*\myG) to[/tikz/circuitikz/bipoles/length=0.8cm, sV, l=$v_1$] ++(0,2*\myG)
	(start)++(\myD,-1*\myG) to[/tikz/circuitikz/bipoles/length=0.8cm, R, l=$v_2$] ++(0,2*\myG)
	;
	%
\end{circuitikz}
